Short Term Blood Glucose Prediction based on Continuous Glucose Monitoring Data

Continuous Glucose Monitoring (CGM) has enabled important opportunities for diabetes management. This study explores the use of CGM data as input for digital decision support tools. We investigate how Recurrent Neural Networks (RNNs) can be used for Short Term Blood Glucose (STBG) prediction and compare the RNNs to conventional time-series forecasting using Autoregressive Integrated Moving Average (ARIMA). A prediction horizon up to 90 min into the future is considered. In this context, we evaluate both population-based and patient-specific RNNs and contrast them to patient-specific ARIMA models and a simple baseline predicting future observations as the last observed. We find that the population-based RNN model is the best performing model across the considered prediction horizons without the need of patient-specific data. This demonstrates the potential of RNNs for STBG prediction in diabetes patients towards detecting/mitigating severe events in the STBG, in particular hypoglycemic events. However, further studies are needed in regards to the robustness and practical use of the investigated STBG prediction models.

==> chapters/temp.tex <==
\begin{table*}[h]
\caption{Overall table for all the model performances in terms of average mae and rmse with corresponding standard error of the mean based on the 7 CGM test days of the 15 patients (CGM training days = 7).}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} &  & \multicolumn{5}{c}{\textbf{MAE (Standard Error) [mmol/L]}} &  & \multicolumn{5}{c}{\textbf{RMSE (Standard Error) [mmol/L]}} \\ \midrule
 &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  & \multicolumn{1}{c}{\textbf{15 min}} & \multicolumn{1}{c}{\textbf{30 min}} & \multicolumn{1}{c}{\textbf{45 min}} & \multicolumn{1}{c}{\textbf{60 min}} & \multicolumn{1}{c}{\textbf{90 min}} &  & \multicolumn{1}{c}{\textbf{15 min}} & \multicolumn{1}{c}{\textbf{30 min}} & \multicolumn{1}{c}{\textbf{45 min}} & \multicolumn{1}{c}{\textbf{60 min}} & \multicolumn{1}{c}{\textbf{90 min}} \\
 &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Population-based LSTM (pretraining)} &  & 0.4392 $\pm$ 0.0282 & 0.8219 $\pm$ 0.0507 & 1.1741 $\pm$ 0.0738 & 1.4919 $\pm$ 0.0980 & 1.9996 $\pm$ 0.1403 &  & 0.6492 $\pm$ 0.0449 & 1.1557 $\pm$ 0.0753 & 1.6191 $\pm$ 0.1067 & 2.0317 $\pm$ 0.1397 & 2.6718 $\pm$ 0.1974 \\
\textbf{Finetuned Patient-specific LSTM (with pretraining)} &  & 0.4406 $\pm$ 0.0297 & 0.8261 $\pm$ 0.0547 & 1.1826 $\pm$ 0.0804 & 1.5049 $\pm$ 0.1066 & 2.0170 $\pm$ 0.1510 &  & 0.6493 $\pm$ 0.0459 & 1.1570 $\pm$ 0.0776 & 1.6218 $\pm$ 0.1107 & 2.0364 $\pm$ 0.1446 & 2.6796 $\pm$ 0.2016 \\
\textbf{Patient-specific LSTM (without pretraining)} &  & 0.4753 $\pm$ 0.0330 & 0.8788 $\pm$ 0.0598 & 1.2406 $\pm$ 0.0842 & 1.5607 $\pm$ 0.1071 & 2.0669 $\pm$ 0.1431 &  & 0.6961 $\pm$ 0.0512 & 1.2374 $\pm$ 0.0882 & 1.7101 $\pm$ 0.1195 & 2.1187 $\pm$ 0.1469 & 2.7415 $\pm$ 0.1881 \\
\textbf{Patient-specific ARIMA} &  & 0.4569 $\pm$ 0.0306 & 0.8587 $\pm$ 0.0558 & 1.2307 $\pm$ 0.0817 & 1.5721 $\pm$ 0.1082 & 2.1241 $\pm$ 0.1542 &  & 0.6782 $\pm$ 0.0483 & 1.2158 $\pm$ 0.0821 & 1.7013 $\pm$ 0.1161 & 2.1358 $\pm$ 0.1500 & 2.8284 $\pm$ 0.2098 \\
\textbf{Last Observation Carried Forward} &  & 0.5650 $\pm$ 0.0356 & 0.9925 $\pm$ 0.0654 & 1.3648 $\pm$ 0.0931 & 1.6901 $\pm$ 0.1185 & 2.2097 $\pm$ 0.1617 &  & 0.8023 $\pm$ 0.0528 & 1.3761 $\pm$ 0.0925 & 1.8662 $\pm$ 0.1284 & 2.2876 $\pm$ 0.1610 & 2.9442 $\pm$ 0.2166 \\
 &  & \multicolumn{5}{l}{} &  & \multicolumn{5}{l}{} \\ \bottomrule
\end{tabular}%
}
\label{tab:res}
\end{table*}
%
